A novel way to determine the scale of inflation

We show that in the Feebly Interacting Massive Particle (FIMP) model of Dark Matter (DM), one may express the inflationary energy scale $H_*$ as a function of three otherwise unrelated quantities, the DM isocurvature perturbation amplitude, its mass and its self-coupling constant, independently of the tensor-to-scalar ratio. The FIMP model assumes that there exists a real scalar particle that alone constitutes the DM content of the Universe and couples to the Standard Model via a Higgs portal. We consider carefully the various astrophysical, cosmological and model constraints, accounting also for variations in inflationary dynamics and the reheating history, to derive a robust estimate for $H_*$ that is confined to a relatively narrow range. We point out that, within the context of the FIMP DM model, one may thus determine $H_*$ reliably even in the absence of observable tensor perturbations.

==> newcommands.tex <==
%edition
%\newcommand{\ie}{\textsl{i.e.~}}
\newcommand{\ie}{{i.e.~}}
\newcommand{\cf}{\textsl{cf.~}}
\newcommand{\eg}{\textsl{e.g.~}}
\newcommand{\etal}{\textsl{et al.~}}
%\newcommand{\apriori}{\textsl{a priori~}}
\newcommand{\apriori}{{a priori~}}
\newcommand{\etc}{\textsl{etc.~}}

%KLD
\newcommand\givenbase[1][]{\:#1\Vert\:}
\let\given\givenbase
\newcommand\sgiven{\givenbase[\delimsize]}



%math function
\newcommand{\mean}[1]{\left\langle #1 \right\rangle}
\newcommand{\order}[1]{\mathcal{O}\!\left(#1\right)}
\newcommand{\Li}[1]{\mathrm{Li}_{#1}}
\DeclareMathOperator{\Ei}{Ei}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
\DeclareMathOperator{\erf}{erf}
\newcommand{\tr}{\mathrm{Tr}}

%larger math symbols
\newcommand{\largemathxl}[1]{{\mathlarger{#1}}}
\newcommand{\largemathxxl}[1]{{\mathlarger{\mathlarger{#1}}}}
\newcommand{\largemathxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{#1}}}}}
\newcommand{\mathlargerxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}
\newcommand{\mathlargerxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}
\newcommand{\mathlargerxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}
\newcommand{\mathlargerxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}}

%alias
\newcommand{\lta}{\lesssim}
\newcommand{\gta}{\gtrsim}
%differential d
\newcommand{\dd}{\mathrm{d}}
%e function
%\newcommand{\ee}{\mathrm{e}}
\newcommand{\ee}{e}


%bold symbols
\newcommand{\boldmu}{\boldsymbol{\mu}}
\newcommand{\boldSigma}{\boldsymbol{\Sigma}}
\newcommand{\boldsigma}{\boldsymbol{\sigma}}


%style
\newcommand{\sss}[1]{{\scriptscriptstyle{#1}}}
\newcommand{\boldmathsymbol}[1]{{\ensuremath{\boldsymbol{#1}}}}

\newcommand{\uPl}{\mathrm{Pl}}
\newcommand{\uin}{\mathrm{in}}
\newcommand{\umin}{\mathrm{min}}
\newcommand{\umax}{\mathrm{max}}
\newcommand{\uend}{\mathrm{end}}
\newcommand{\uini}{\mathrm{ini}}
\newcommand{\ueff}{\mathrm{eff}}
\newcommand{\uinf}{\mathrm{inf}}
\newcommand{\ureh}{\mathrm{reh}}
\newcommand{\uereh}{\mathrm{ereh}}
\newcommand{\urad}{\mathrm{rad}}
\newcommand{\utop}{\mathrm{top}}
\newcommand{\ucri}{\mathrm{cri}}
\newcommand{\ucl}{\mathrm{cl}}
\newcommand{\unuc}{\mathrm{nuc}}
\newcommand{\uobs}{\mathrm{obs}}
\newcommand{\ulim}{\mathrm{lim}}
\newcommand{\uphys}{\mathrm{phys}}
\newcommand{\uPgiP}{\mathrm{(gi)}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\uc}{\mathrm{c}}
\newcommand{\ub}{\mathrm{b}}
\newcommand{\us}{\mathrm{s}}
\newcommand{\uS}{\mathrm{S}}
\newcommand{\uM}{\mathrm{M}}
\newcommand{\uPSP}{(\uS)}
\newcommand{\uV}{\mathrm{V}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uPTP}{(\uT)}
\newcommand{\uE}{\mathrm{E}}
\newcommand{\usssTE}{\sss{\uT \uE}}
\newcommand{\usssS}{\sss{\uS}}
\newcommand{\usssPSP}{\sss{\uPSP}}
\newcommand{\usssT}{\sss{\uT}}
\newcommand{\usssPTP}{\sss{\uPTP}}
\newcommand{\usssPMoneP}{\sss{(\uM=1)}}
\newcommand{\usssPl}{\sss{\uPl}}
\newcommand{\usssRH}{\ureh}
\newcommand{\usssV}{\sss{\uV}}
\newcommand{\usssE}{\sss{\uE}}
\newcommand{\nS}{n_\usssS}
\newcommand{\nT}{n_\usssT}
\newcommand{\alphaS}{\alpha_\usssS}
\newcommand{\alphaT}{\alpha_\usssT}
\newcommand{\zero}{{_0}}
\newcommand{\one}{{_1}}
\newcommand{\two}{{_2}}
\newcommand{\udm}{\mathrm{dm}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\muS}{\mu_\usssS}
\newcommand{\muT}{\mu_\usssT}
\newcommand{\muST}{\mu_{\usssS,\usssT}}
\newcommand{\uRL}{\mathrm{RL}}
\newcommand{\uNL}{\mathrm{NL}}
\newcommand{\uwkb}{\mathrm{WKB}}

\newcommand{\bmk}{\boldmathsymbol{k}}
\newcommand{\bmx}{\boldmathsymbol{x}}

\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calM}{\mathcal{M}}

\newcommand{\setR}{\mathbb{R}}
\newcommand{\setC}{\mathbb{C}}

\newcommand{\Rea}{\Re \mathrm{e}\,}
\newcommand{\Ima}{\Im \mathrm{m}\,}
\newcommand{\like}{{\cal L}}

%Planck posterior
\newcommand{\pPl}{p_{{}_{\uPl}}}
% fiducal mu
\newcommand{\bmuf}{\boldsymbol{\mu}_{{}_{\rm F}}}
\newcommand{\bmubeta}{\boldsymbol{\mu}_{\beta}}
\newcommand{\bmugamma}{\boldsymbol{\mu}_{\gamma}}
\newcommand{\muf}{\mu_{{}_{{\rm F}}}}
\newcommand{\mubeta}{\mu_{\beta}}
\newcommand{\mugamma}{\mu_{\gamma}}
\newcommand{\boldsig}{\boldsymbol{\sigma}}

%units
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\km}{\mathrm{km}}
\renewcommand{\sec}{\mathrm{s}}
\newcommand{\pc}{\mathrm{pc}}
\newcommand{\kpc}{\mathrm{kpc}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\K}{\mathrm{K}}

\newcommand{\boldx}{\boldsymbol{x}}
\newcommand{\boldy}{\boldsymbol{y}}

% General Cosmology

\newcommand{\Hu}{\mathcal{H}}
\newcommand{\Ka}{\mathcal{K}}
\newcommand{\Zed}{\mathcal{Z}}
\newcommand{\cs}{c_{_\mathrm{S}}}

%cosmo
\newcommand{\omegaT}{\omega_\usssT}
\newcommand{\omegaS}{\omega_\usssS}
\newcommand{\omegaST}{\omega_{\usssS, \usssT}}
\newcommand{\OmegaL}{\Omega_\Lambda}
\newcommand{\OmegaCDM}{\Omega_\udm}
\newcommand{\OmegaB}{\Omega_\ub}
\newcommand{\OmegaR}{\Omega_\gamma}
\newcommand{\Qrms}{Q_{\mathrm{rms-PS}}}
\newcommand{\wstate}{w}
\newcommand{\Mc}{M_\uc}
\newcommand{\potS}{U_{_\uS}}
\newcommand{\potT}{U_{_\uT}}

\newcommand{\mpl}{m_\usssPl}
\newcommand{\Mp}{M_\usssPl}


%inflation
\newcommand{\Hzero}{H_0}
\newcommand{\Hstar}{H_*}
\newcommand{\kstar}{k_*}
\newcommand{\Pstar}{P_*}
\newcommand{\astar}{a_*}
\newcommand{\Pnum}{P^{\usssPMoneP}}
\newcommand{\calNnuc}{\mathcal{N}^\unuc}
\newcommand{\calNend}{\mathcal{N}^\uend}
\newcommand{\calFnuc}{\mathcal{F}^\unuc}
\newcommand{\calFend}{\mathcal{F}^\uend}
\newcommand{\rRL}{r_\uRL}
\newcommand{\fnl}{f_\uNL}
\newcommand{\csini}{c_{\us \uini}}

\newcommand{\etastar}{\eta_*}
\newcommand{\nustar}{\nu_*}
\newcommand{\csstar}{c_{\us*}}
\newcommand{\epsonestar}{\epsilon_{1*}}
\newcommand{\epstwostar}{\epsilon_{2*}}
\newcommand{\epsthreestar}{\epsilon_{3*}}
\newcommand{\deltaonestar}{\delta_{1*}}
\newcommand{\deltatwostar}{\delta_{2*}}
\newcommand{\epsnstar}{\epsilon_{n*}}
\newcommand{\epsnponestar}{\epsilon_{n+1*}}
\newcommand{\xstar}{x_*}
\newcommand{\deci}{\mathscr{D}}

\newcommand{\ustar}{u_*}
\newcommand{\wstar}{w_*}

\newcommand{\dia}{\sss{\diamond}}
\newcommand{\Hdia}{H_\dia}
\newcommand{\kdia}{k_\dia}
\newcommand{\etadia}{\eta_\dia}
\newcommand{\csdia}{c_{\us \dia}}
\newcommand{\epsonedia}{\epsilon_{1\dia}}
\newcommand{\epstwodia}{\epsilon_{2\dia}}
\newcommand{\epsthreedia}{\epsilon_{3\dia}}
\newcommand{\epsfourdia}{\epsilon_{4\dia}}
\newcommand{\epsfivedia}{\epsilon_{5\dia}}

\newcommand{\deltaonedia}{\delta_{1\dia}}
\newcommand{\deltatwodia}{\delta_{2\dia}}
\newcommand{\deltathreedia}{\delta_{3\dia}}
\newcommand{\deltafourdia}{\delta_{4\dia}}

\newcommand{\grav}{\star}
\newcommand{\Hgrav}{H_\grav}
\newcommand{\kgrav}{k_\grav}
\newcommand{\etagrav}{\eta_\grav}
\newcommand{\epsonegrav}{\epsilon_{1\grav}}
\newcommand{\epstwograv}{\epsilon_{2\grav}}

\newcommand{\aH}{\sss{\circledast}}
\newcommand{\kah}{k_\aH}
\newcommand{\etaah}{\eta_\aH}

\newcommand{\Dwkb}{D_{_\uwkb}}
\newcommand{\Awkb}{A_{_\uwkb}}
%\newcommand{\etaH}{\eta_{_{H}}}

\newcommand{\pisto}{\pi_\mathrm{sto}}

%efolds
\newcommand{\efolds}{$e$-folds~}
\newcommand{\efold}{$e$-fold}
\newcommand{\Nini}{N_\uini}
\newcommand{\Nend}{N_\uend}
\newcommand{\Nreh}{N_\ureh}
\newcommand{\Nstar}{N_*}
\newcommand{\Nzero}{N_\zero}
\newcommand{\Nstarnuc}{N_*^\unuc}
\newcommand{\Nstarend}{N_*^\uend}

%begin and end equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}


%figures size
\newlength{\wsingfig}
\setlength{\wsingfig}{0.99\textwidth}
\newlength{\wdblefig}
\setlength{\wdblefig}{0.49\textwidth}
\newlength{\wquadfig}
\setlength{\wquadfig}{0.249\textwidth}
\newlength{\wtriplefig}
\setlength{\wtriplefig}{0.333\textwidth}


% References
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[1]{Eqs.~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~{\ref{#1}}}
\newcommand{\Figs}[1]{Figs.~{\ref{#1}}}
\newcommand{\Ref}[1]{Ref.~{\cite{#1}}}
\newcommand{\Refs}[1]{Refs.~{\cite{#1}}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Secs}[1]{Secs.~\ref{#1}}
\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\Apps}[1]{Appendixes.~\ref{#1}}
